Distributive Dynamic Spectrum Access through Deep Reinforcement Learning: A Reservoir Computing Based Approach

Dynamic spectrum access (DSA) is regarded as an effective and efficient technology to share radio spectrum among different networks. As a secondary user (SU), a DSA device will face two critical problems: avoiding causing harmful interference to primary users (PUs), and conducting effective interference coordination with other secondary users. These two problems become even more challenging for a distributed DSA network where there is no centralized controllers for SUs. In this paper, we investigate communication strategies of a distributive DSA network under the presence of spectrum sensing errors. To be specific, we apply the powerful machine learning tool, deep reinforcement learning (DRL), for SUs to learn "appropriate" spectrum access strategies in a distributed fashion assuming NO knowledge of the underlying system statistics. Furthermore, a special type of recurrent neural network (RNN), called the reservoir computing (RC), is utilized to realize DRL by taking advantage of the underlying temporal correlation of the DSA network. Using the introduced machine learning-based strategy, SUs could make spectrum access decisions distributedly relying only on their own current and past spectrum sensing outcomes. Through extensive experiments, our results suggest that the RC-based spectrum access strategy can help the SU to significantly reduce the chances of collision with PUs and other SUs. We also show that our scheme outperforms the myopic method which assumes the knowledge of system statistics, and converges faster than the Q-learning method when the number of channels is large.

==> Algorithms/QLearing.tex <==
\begin{algorithm}  
\caption{Q-learning}
\label{alg:QLearning}
\begin{algorithmic}  
\STATE {Initialize $Q(s,a)$ arbitrarily}
\STATE {Initialize $s$} 
\REPEAT
\STATE {1. Choose $a_t$ from $s_t$ using policy derived from $Q$}
\STATE {2. Take action $a_t$, receive $r_{t+1}$, observe $s_{t+1}$}
\STATE {3. Update Q-value}
\STATE {
\begin{displaymath}
\begin{split}
Q(s_t,a_t) &= Q(s_t,a_t) \\
&+ \alpha[ r_{t+1} 
+ \gamma \max_{a_{t+1}}{Q(s_{t+1},a_{t+1})} - Q(s_t,a_t)]
\end{split}
\end{displaymath}
}
\STATE {4. $s_t = s_{t+1}$}
\UNTIL{s is terminal} 
\end{algorithmic}  
\end{algorithm}  

==> IOT final/Algorithms/DQN_training.tex <==
\begin{algorithm}
\caption{DQN training process}
\label{alg:DQN_training}
\begin{algorithmic}
\STATE {
1) Initialize $\text{DQN}_{\text{t}}^l$ and $\text{DQN}_{\text{e}}^l$ with the same structure and initial weights for each SU $l$.}\\

2) Each SU $l$ inputs $S^l(t)$ to $\text{DQN}_{\text{e}}^l$ and chooses the action $a^l(t)$ based on Equation~\ref{eq:epsilon greedy}.

3) Each SU $l$ gets a reward $r_{t+1}^l$, and observes the next state $S^l(t+1)$.

4) Store $S^l(t), a^l(t), r^l(t+1), S^l(t+1)$ and replace $S^l(t)$ with $S^l(t+1)$.

5) Repeats step 2 to step 4 for $T$ times at $T$ slots.

6) Given the stored $T$ sequences, $S^l(t), a^l(t), r^l(t+1), S^l(t+1)$, input $S^l(t)$ and $S^l(t+1)$ to $\text{DQN}_{\text{e}}^l$ and $\text{DQN}_{\text{t}}^l$ to generate $\text{Q}_{\text{e}}^l(S^l(t), a)$ and $\text{Q}_{\text{t}}^l(S^l(t+1), a)$, respectively. Then update the $\text{DQN}_{\text{e}}^l(a)$ to minimize the mean-square-error of the following function:
\begin{equation*}
[r^l(t+1) + \gamma \max_{a}{\text{Q}_{\text{t}}^l(S^l(t+1),a)} - \text{Q}_{\text{e}}(S^l(t),a^l(t))]^2
\end{equation*}

8) Replace $\text{DQN}_{\text{t}}^l$ with $\text{DQN}_{\text{e}}^l$:


\end{algorithmic}
\end{algorithm}

==> IOT final/Algorithms/QLearing.tex <==
\begin{algorithm}  
\caption{Q-learning}
\label{alg:QLearning}
\begin{algorithmic}  
\STATE {Initialize $Q(s,a)$ arbitrarily}
\STATE {Initialize $s$} 
\REPEAT
\STATE {1. Choose $a_t$ from $s_t$ using policy derived from $Q$}
\STATE {2. Take action $a_t$, receive $r_{t+1}$, observe $s_{t+1}$}
\STATE {3. Update Q-value}
\STATE {
\begin{displaymath}
\begin{split}
Q(s_t,a_t) &= Q(s_t,a_t) \\
&+ \alpha[ r_{t+1} 
+ \gamma \max_{a_{t+1}}{Q(s_{t+1},a_{t+1})} - Q(s_t,a_t)]
\end{split}
\end{displaymath}
}
\STATE {4. $s_t = s_{t+1}$}
\UNTIL{s is terminal} 
\end{algorithmic}  
\end{algorithm}  

==> IOT final/Figures/architecture.tex <==
\begin{figure*}[t]
\centering
	\includegraphics[width=.73\linewidth]{Figures/architecture.jpg}
	\caption{Architecture for distributive deep reinforcement learning.}
	\label{fig:architecture}
\end{figure*}

==> IOT final/Figures/framework.tex <==
\begin{figure}[t]
\centering
	\includegraphics[width=1.0\linewidth]{Figures/Framework.jpeg}
	\caption{System Model.}
	\label{fig:framework}
\end{figure}

==> IOT final/Figures/geometry_channel22_su1.tex <==
\begin{figure}[ht]
\centering
	\includegraphics[width=.75\linewidth]{Figures/geometry_channel22_su1.jpg}
	\caption{DSA Network Geometry (No. of channel = 22 and No. of SU = 1)}
	\label{fig:geometry_channel22_su1}
\end{figure}

==> IOT final/Figures/geometry_channel6_su2_punish_-2.tex <==
\begin{figure}[ht]
\centering
	\includegraphics[width=.75\linewidth]{Figures/geometry_channel6_su2_punish_-2.jpg}
	\caption{DSA Network Geometry (No. of channel = 6 and No. of SU = 2)}
	\label{fig:geometry_channel6_su2_punish_-2}
\end{figure}

==> IOT final/Figures/learning_procedure.tex <==
\begin{figure}[t]
\centering
	\includegraphics[width=.7\linewidth]{Figures/learning_procedure.jpg}
	\caption{Learning procedure in DSA.}
	\label{fig:learning_procedure}
\end{figure}

==> IOT final/Figures/reservoir_computing.tex <==
\begin{figure}[t]
\centering
	\includegraphics[width=.9\linewidth]{Figures/reservoir_computing.jpg}
	\caption{Reservoir Computing.}
	\label{fig:reservoir_computing}
\end{figure}

==> IOT final/Figures/result_channel6_su2_punish_-2.tex <==
\begin{figure}[ht]
\centering
	\includegraphics[width=.95\linewidth]{Figures/result_channel6_su2_punish_-2.jpg}
	\caption{The average success number, collision number with PUs, collision number with SUs, and reward with the training time (No. of channel = 6 and No. of SU = 2)}
	\label{fig:result_channel6_su2_punish_-2}
\end{figure}

==> IOT final/Figures/result_channel_1_su_1.tex <==
\begin{figure}[ht]
\centering
	\includegraphics[width=.95\linewidth]{Figures/result_channel1_su1.jpg}
	\caption{The average success number, collision number with PUs, and reward with the training time (No. of channel = 1 and No. of SU = 1)}
	\label{fig:result_channel_1_su_1}
\end{figure}

==> IOT final/Figures/result_channel_22_su_1.tex <==
\begin{figure}[ht]
\centering
	\includegraphics[width=.95\linewidth]{Figures/result_channel22_su1.jpg}
	\caption{The average success number, collision number with PUs, and reward with the training time (No. of channel = 22 and No. of SU = 1)}
	\label{fig:result_channel_22_su_1}
\end{figure}

==> IOT final/Figures/two_state_markov_chain.tex <==
\begin{figure}[t]
\centering
	\includegraphics[width=.9\linewidth]{Figures/two_state_markov_chain.jpg}
	\caption{Two-state Markov chain.}
	\label{fig:two_state_markov_chain}
\end{figure}

==> IOT final/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> IOT final/Tables/channel_model_parameters.tex <==
\begin{table}
	\centering
	\caption{Channel model paramters}
	\label{tab:channel_model_parameters}  
	\begin{tabular}{|c|c|}
	\hline
	SU transmit power & 20mW \\ \hline
    PU transmit power & 40mW \\ \hline
    $f_c$ & 5GHz \\ \hline
    $\overline {PL}$ & 41 \\ \hline
    $A_W$ & 22.7 \\ \hline
    $B_W$ & 20 \\ \hline
    $\kappa$ & 8 \\ \hline
    $B$ & 1MHz \\ \hline
    $N_0$ & $10^{-14.7}$(mW/Hz) \\ \hline
    \end{tabular}
\end{table}



==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************

